Differentiable Black-box and Gray-box Modeling of Nonlinear Audio Effects

Audio effects are extensively used at every stage of audio and music content creation. The majority of differentiable audio effects modeling approaches fall into the black-box or gray-box paradigms; and most models have been proposed and applied to nonlinear effects like guitar amplifiers, overdrive, distortion, fuzz and compressor. Although a plethora of architectures have been introduced for the task at hand there is still lack of understanding on the state of the art, since most publications experiment with one type of nonlinear audio effect and a very small number of devices. In this work we aim to shed light on the audio effects modeling landscape by comparing black-box and gray-box architectures on a large number of nonlinear audio effects, identifying the most suitable for a wide range of devices. In the process, we also: introduce time-varying gray-box models and propose models for compressor, distortion and fuzz, publish a large dataset for audio effects research - ToneTwist AFx https://github.com/mcomunita/tonetwist-afx-dataset - that is also the first open to community contributions, evaluate models on a variety of metrics and conduct extensive subjective evaluation. Code https://github.com/mcomunita/nablafx and supplementary material https://github.com/mcomunita/nnlinafx-supp-material are also available.

==> TABLES/_table_results_single-fx-val-test-loss.tex <==
% \vspace{-0.3cm}
\setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{0.85}
\begin{table*}[h]
    \centering
    \small
    \caption{\textit{Normalized L1 and MR-STFT for non parametric amp model: Custom Dynamic Fuzz}}
    % \hspace*{-0cm}
    \begin{tabular}{lccccccccccccc}
        \toprule
        \multirow{2}{*}{Model}
            & \multirow{2}{*}{Params.}
                & \multirow{2}{*}{LR}
                    & \multicolumn{2}{c}{Weights}
                        & \multicolumn{3}{c}{Val. Loss}
                            & \multicolumn{3}{c}{Test Loss} \\ 
        \cmidrule(lr){4-5} 
            \cmidrule(lr){6-8} 
                \cmidrule(lr){9-11}
        &   &   & $L1$ & MR-STFT & Tot. & $L1$ & MR-STFT & Tot. & $L1$ & MR-STFT \\ 
        \midrule
        LSTM-32
            & 4.5k  & - & - & - & - & - & - & - & - & - & \\
        LSTM-96       
            & 38.1k & - & - & - & - & - & - & - & - & - & \\
        % \midrule
        % LSTM-TVC-32
        %     & - & - & - & - & - & - & - & - & - \\
        % LSTM-TVC-96
        %     & - & - & - & - & - & - & - & - & - \\
        \midrule
        TCN-45-S-16               
            & 7.5k & .005 & - & - & - & - & - & - & - & - & \\ 
        TCN-45-L-16               
            & 7.3k & .005 & - & - & - & - & - & - & - & -  \\
        TCN-250-S-16               
            & 14.5k & .005 & - & - & - & - & - & - & - & - \\ 
        TCN-250-L-16               
            & 18.4k & .005 & - & - & - & - & - & - & - & - \\
        TCN-2500-S-16               
            & 13.7k & .005 & - & - & - & - & - & - & - & - \\ 
        TCN-2500-L-16               
            & 11.9k & .005 & - & - & - & - & - & - & - & - \\
        \midrule
        TCN-TF-45-S-16               
            & 39.5k & .005 & - & - & - & - & - & - & - & - \\
        TCN-TF-45-L-16               
            & 71.3k & .005 & - & - & - & - & - & - & - & - \\
        TCN-TF-250-S-16               
            & 52.9k & .005 & - & - & - & - & - & - & - & - \\
        TCN-TF-250-L-16               
            & 88.8k & .005 & - & - & - & - & - & - & - & - \\
        TCN-TF-2500-S-16               
            & 45.7k & .005 & - & - & - & - & - & - & - & - \\
        TCN-TF-2500-L-16               
            & 75.9k & .005 & - & - & - & - & - & - & - & - \\
        % \midrule
        % TCN-TTF-45-S-16               
        %     & - & - & - & - & - & - & - & - & - \\
        % TCN-TTF-45-L-16               
        %     & - & - & - & - & - & - & - & - & - \\
        % \midrule
        % TCN-TVF-45-S-16               
        %     & - & - & - & - & - & - & - & - & - \\
        % TCN-TVF-45-L-16               
        %     & - & - & - & - & - & - & - & - & - \\
        \midrule
        GCN-45-S-16               
            & 16.2k & .005 & - & - & - & - & - & - & - & - \\ 
        GCN-45-L-16               
            & 17.1k & .005 & - & - & - & - & - & - & - & - \\
        GCN-250-S-16               
            & 30.4k & .005 & - & - & - & - & - & - & - & - \\ 
        GCN-250-L-16               
            & 39.6k & .005 & - & - & - & - & - & - & - & - \\
        GCN-2500-S-16               
            & 28.6k & .005 & - & - & - & - & - & - & - & - \\ 
        GCN-2500-L-16               
            & 26.4k & .005 & - & - & - & - & - & - & - & - \\
        \midrule
        GCN-TF-45-S-16               
            & 141k & .005 & - & - & - & - & - & - & - & - \\
        GCN-TF-45-L-16               
            & 268k & .005 & - & - & - & - & - & - & - & - \\
        GCN-TF-250-S-16               
            & 180k & .005 & - & - & - & - & - & - & - & - \\
        GCN-TF-250-L-16               
            & 315k & .005 & - & - & - & - & - & -& - & -  \\
        GCN-TF-2500-S-16               
            & 154k & .005 & - & - & - & - & - & - & - & - \\
        GCN-TF-2500-L-16               
            & 277k & .005 & - & - & - & - & - & - & - & - \\
        % \midrule
        % GCN-TTF-45-S-16               
        %     & - & - & - & - & - & - & - & - & - \\
        % GCN-TTF-45-L-16               
        %     & - & - & - & - & - & - & - & - & - \\
        % \midrule
        % GCN-TVF-45-S-16               
        %     & - & - & - & - & - & - & - & - & - \\
        % GCN-TVF-45-L-16               
        %     & - & - & - & - & - & - & - & - & - \\
        \midrule
        S4-B4-S4-C16              
            & 2.4k & .01 & - & - & - & - & - & - & - & - \\
        S4-B8-S32-C16               
            & 19k & .01 & - & - & - & - & - & - & - & - \\
        \midrule
        S4-TF-B4-S4-C16              
            & 28k & .01 & - & - & - & - & - & - & - & - \\
        S4-TF-B8-S32-C16               
            & 70.2k & .01 & - & - & - & - & - & - & - & - \\
        \midrule
        GB-DIST-MLP             
            & 2.2k & .1 (.01) & - & - & - & - & - & - & - & - \\
        GB-DIST-RNL             
            & 47 & .1 (1) & - & - & - & - & - & - & - & - \\
        \midrule
        GB-DIST-MLP-FIR
            & 6.6k & .1 (.01/.01) & - & - & - & - & - & - & - & - \\
        GB-DIST-RNL-FIR         
            & 4.4k & .1 (1/.01) & - & - & - & - & - & - & - & - \\
        \midrule
        GB-FUZZ-MLP             
            & 2.3k & .1 (.01) & - & - & - & - & - & - & - & - \\
        GB-FUZZ-RNL             
            & 62 & .1 (1) & - & - & - & - & - & - & - & - \\
        \midrule
        GB-FUZZ-MLP-FIR
            & 6.6k & .1 (.01/.01) & - & - & - & - & - & - & - & - \\
        GB-FUZZ-RNL-FIR         
            & 4.4k & .1 (1/.01) & - & - & - & - & - & - & - & - \\
        \midrule
        GB-COMP
            & 47 & - & - & - & - & - & - & - & - & - \\
        \bottomrule 
    \end{tabular}
    \label{tab:other_fx}
\end{table*}

==> TABLES/correlation_subj-eval-vs-fad.tex <==
%\setlength{\tabcolsep}{3.8pt}
% \vspace{-0.3cm}
% \renewcommand{\arraystretch}{0.85}
\begin{table*}[h]
    \small
    \caption{Spearman correlation ($\rho$) and $p$-value ($<0.05$) between subjective ratings and objective metrics for each device type and overall. Correlation is negative since low metrics values correspond to high ratings values. Bold indicates highest absolute value.}
    \label{tab:results_overall}
    \centerline{
        \begin{tabular}{lcccccccccc} 
            \midrule
            \midrule
            \multirow{2}{*}{Effect Type} 
            & \multicolumn{2}{c}{FAD$_{\text{VGGish}}$} 
            &  \multicolumn{2}{c}{FAD$_{\text{PANN}}$} 
            & \multicolumn{2}{c}{FAD$_{\text{CLAP}}$} 
            & \multicolumn{2}{c}{FAD$_{\text{AFx-Rep}}$} \\
            
            \cmidrule(lr){2-3} 
            \cmidrule(lr){4-5} 
            \cmidrule(lr){6-7} 
            \cmidrule(lr){8-9}
            \cmidrule(lr){10-11}
            
            & $\rho$ & $p$ 
            & $\rho$ & $p$ 
            & $\rho$ & $p$ 
            & $\rho$ & $p$ \\ 
            
            \midrule
            Comp./Limit. & -0.188 & \ding{51} & -0.193 & \ding{51} & -0.172 & \ding{51} & \textbf{-0.194} & \ding{51} \\
            Overdrive & -0.207 & \ding{51} & -0.061 & \ding{55} & -0.182 & \ding{51} & \textbf{-0.211} & \ding{51} \\
            Distortion & -0.592 & \ding{51} & -0.404 & \ding{51} & \textbf{-0.613} & \ding{51} & -0.533 & \ding{51} \\
            Fuzz & \textbf{-0.511} & \ding{51} & -0.314 & \ding{51} & -0.434 & \ding{51} & -0.482 & \ding{51} \\
            \midrule
            Overall & \textbf{-0.430} & \ding{51} & -0.303 & \ding{51} & -0.406 & \ding{51} & -0.417 & \ding{51} \\
            \midrule
            \midrule
        \end{tabular} 
    }
    % \vspace{-0.0cm}
    % \vspace{0.2cm}
\end{table*}

==> TABLES/correlation_subj-eval-vs-metrics.tex <==
%\setlength{\tabcolsep}{3.8pt}
% \vspace{-0.3cm}
% \renewcommand{\arraystretch}{0.85}
\begin{table*}[h]
    \small
    \caption{Spearman correlation ($\rho$) and $p$-value ($<0.05$) between subjective ratings and objective metrics for each device type and overall. Correlation is negative since low metrics values correspond to high ratings values. Bold indicates highest absolute value.}
    \label{tab:results_overall}
    \centerline{
        \begin{tabular}{lcccccccccc} 
            \midrule
            \midrule
            \multirow{2}{*}{Effect Type} 
                & \multicolumn{2}{c}{L1} 
                    &  \multicolumn{2}{c}{MR-STFT} 
                        & \multicolumn{2}{c}{MSE} 
                            & \multicolumn{2}{c}{ESR} 
                                & \multicolumn{2}{c}{MAPE} \\
            \cmidrule(lr){2-3} 
                \cmidrule(lr){4-5} 
                    \cmidrule(lr){6-7} 
                        \cmidrule(lr){8-9}
                            \cmidrule(lr){10-11}
                                % \cmidrule(lr){13-14}
            & $\rho$ & $p$ & $\rho$ & $p$ & $\rho$ & $p$ & $\rho$ & $p$ & $\rho$ & $p$ \\ 
            \midrule
            Comp./Limit. 
                & \textbf{-0.188} & \ding{51} 
                & -0.158 & \ding{51} 
                & -0.185* & \ding{51} 
                & -0.149 & \ding{55} 
                & -0.152 & \ding{55}\\
            Overdrive 
                & -0.183 & \ding{51} 
                & -0.277* & \ding{51} 
                & -0.171 & \ding{51} 
                & -0.264 & \ding{51} 
                & \textbf{-0.361} & \ding{51}\\
            Distortion 
                & -0.242 & \ding{51} 
                & \textbf{-0.536} & \ding{51} 
                & -0.267 & \ding{51} 
                & -0.389* & \ding{51} 
                & -0.214 & \ding{51}\\
            Fuzz 
                & -0.424 & \ding{51} 
                & \textbf{-0.488} & \ding{51} 
                & -0.406 & \ding{51} 
                & -0.470* & \ding{51} 
                & -0.453 & \ding{51} \\
            \midrule
            Overall 
                & -0.332 & \ding{51} 
                & \textbf{-0.427} & \ding{51} 
                & -0.314 & \ding{51} 
                & -0.311 & \ding{51} 
                & -0.339* & \ding{51} \\
            \midrule
            \midrule
        \end{tabular}
    }
    % \vspace{-0.0cm}
    % \vspace{0.2cm}
\end{table*}

==> TABLES/fad_overall.tex <==
%\setlength{\tabcolsep}{3.8pt}
% \vspace{-0.3cm}
% \renewcommand{\arraystretch}{0.85}
\begin{table*}[h]
    \scriptsize
    \centerline{
        \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|} 
            \midrule
            \midrule
            \multirow{2}{*}{Model} 
                % & \multirow{2}{*}{Params.} 
                    & \multicolumn{2}{c}{Tot. Loss} 
                        & \multicolumn{2}{c}{FAD\textsubscript{VGGish}} 
                            &  \multicolumn{2}{c}{FAD\textsubscript{PANN}} 
                                & \multicolumn{2}{c}{FAD\textsubscript{CLAP}} 
                                    & \multicolumn{2}{c}{FAD\textsubscript{AFX-REP}} \\
                                        % & \multicolumn{2}{c}{Overall} \\
            \cmidrule(lr){2-3} 
                \cmidrule(lr){4-5} 
                    \cmidrule(lr){6-7} 
                        \cmidrule(lr){8-9}
                            \cmidrule(lr){10-11}
                                % \cmidrule(lr){13-14}
            & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ \\ 
            \midrule
            LSTM-32 & 1.0239 & 0.7904 & \underline{2.6187} & 3.6474 & \underline{1.566E-04} & \underline{3.752E-04} & \underline{0.1267} & \underline{0.1437} & 0.2665 & 0.3115 \\ 
            LSTM-96 & 0.8909 & 0.7308 & 2.3226 & \underline{3.7729} & 8.170E-05 & 1.439E-04 & 0.1042 & 0.1183 & 0.2399 & \underline{0.3183} \\ 
            \midrule
            TCN-45-S-16 & 0.7582 & 0.3012 & 0.4986 & 0.3746 & 5.412E-05 & 8.496E-05 & 0.0502 & 0.0468 & 0.1188 & 0.1130 \\ 
            TCN-45-L-16 & 0.7246 & 0.2537 & 0.4024 & 0.2837 & 4.244E-05 & 6.015E-05 & 0.0424 & 0.0420 & 0.1014 & 0.1113 \\ 
            TCN-250-S-16 & 0.6904 & 0.2625 & 0.4168 & 0.3117 & 4.127E-05 & 5.422E-05 & 0.0391 & 0.0333 & 0.1097 & 0.1294 \\ 
            TCN-250-L-16 & 0.6461 & 0.2418 & 0.3248 & 0.2868 & 2.546E-05 & 3.563E-05 & 0.0334 & 0.0348 & 0.0840 & 0.1303 \\ 
            TCN-2500-S-16 & 0.7573 & 0.3142 & 0.5320 & 0.4165 & 4.186E-05 & 3.841E-05 & 0.0426 & 0.0389 & 0.1356 & 0.1549 \\ 
            TCN-2500-L-16 & 0.6390 & 0.2350 & 0.3489 & 0.2967 & 2.365E-05 & 3.187E-05 & 0.0303 & 0.0314 & 0.0873 & 0.1238 \\ 
            \midrule
            TCN-TF-45-S-16 & 0.5793 & 0.2272 & 0.4497 & 0.5686 & 4.408E-05 & 9.285E-05 & 0.0349 & 0.0301 & 0.0690 & 0.0636 \\ 
            TCN-TF-45-L-16 & 0.5237 & \textbf{0.2008} & 0.3201 & 0.4353 & 3.124E-05 & 7.584E-05 & 0.0256 & 0.0258 & 0.0544 & 0.0418 \\ 
            TCN-TF-250-S-16 & 0.5390 & 0.2106 & 0.3142 & 0.3776 & 3.289E-05 & 7.271E-05 & 0.0245 & \textbf{0.0210} & 0.0585 & 0.0519 \\ 
            TCN-TF-250-L-16 & 0.5097 & 0.2029 & 0.2860 & 0.3367 & 2.188E-05 & 5.471E-05 & 0.0262 & 0.0300 & 0.0555 & 0.0831 \\ 
            TCN-TF-2500-S-16 & 0.6026 & 0.2454 & 0.3725 & 0.3766 & 3.887E-05 & 5.643E-05 & 0.0252 & 0.0213 & 0.0892 & 0.1102 \\ 
            TCN-TF-2500-L-16 & 0.5307 & 0.2146 & 0.4338 & 0.8216 & 6.768E-05 & 1.846E-04 & 0.0270 & 0.0310 & 0.0757 & 0.1240 \\ 
            \midrule
            GCN-45-S-16 & 0.6947 & 0.2705 & 0.3742 & 0.3674 & 1.566E-05 & 2.600E-05 & 0.0374 & 0.0397 & 0.1126 & 0.1424 \\ 
            GCN-45-L-16 & 0.6579 & 0.2514 & 0.3337 & 0.3482 & 8.867E-06 & 1.504E-05 & 0.0363 & 0.0383 & 0.0879 & 0.1341 \\ 
            GCN-250-S-16 & 0.6289 & 0.2674 & 0.3101 & 0.3311 & 1.587E-05 & 3.820E-05 & 0.0300 & 0.0292 & 0.0795 & 0.1371 \\ 
            GCN-250-L-16 & 0.5950 & 0.2521 & 0.3155 & 0.3339 & 1.436E-05 & 2.681E-05 & 0.0313 & 0.0328 & 0.0646 & 0.1229 \\ 
            GCN-2500-S-16 & 0.6273 & 0.2655 & 0.3582 & 0.3970 & 2.080E-05 & 3.638E-05 & 0.0296 & 0.0322 & 0.0842 & 0.1743 \\ 
            GCN-2500-L-16 & 0.5757 & 0.2395 & 0.3056 & 0.3099 & 1.047E-05 & 2.048E-05 & 0.0284 & 0.0308 & 0.0613 & 0.0827 \\ 
            \midrule
            GCN-TF-45-S-16 & 0.5393 & 0.2276 & 0.3205 & 0.3834 & 2.016E-05 & 4.763E-05 & 0.0293 & 0.0277 & 0.0665 & 0.0680 \\ 
            GCN-TF-45-L-16 & 0.4868 & 0.2067 & 0.2881 & 0.3997 & 3.470E-05 & 1.039E-04 & 0.0251 & 0.0263 & 0.0337 & 0.0368 \\ 
            GCN-TF-250-S-16 & 0.5500 & 0.2659 & 0.3183 & 0.3734 & 2.869E-05 & 7.653E-05 & 0.0301 & 0.0340 & 0.0666 & 0.0816 \\ 
            GCN-TF-250-L-16 & 0.5109 & 0.2349 & 0.3067 & 0.3881 & 4.108E-05 & 8.833E-05 & 0.0259 & 0.0262 & 0.0547 & 0.0756 \\ 
            GCN-TF-2500-S-16 & 0.5385 & 0.2209 & 0.3185 & 0.4586 & 1.854E-05 & 4.484E-05 & 0.0218 & 0.0212 & 0.0528 & 0.0616 \\ 
            GCN-TF-2500-L-16 & 0.4867 & 0.2072 & 0.2989 & 0.4172 & 3.024E-05 & 8.663E-05 & 0.0231 & 0.0286 & 0.0326 & 0.0323 \\ 
            \midrule
            S4-S-16 & 0.5699 & 0.2523 & 0.2452 & 0.2640 & 8.715E-06 & 1.692E-05 & 0.0241 & 0.0287 & 0.0643 & 0.1184 \\ 
            S4-L-16 & 0.4627 & 0.2269 & \textbf{0.1702} & \textbf{0.2169} & \textbf{6.061E-06} & \textbf{8.751E-06} & \textbf{0.0185} & 0.0241 & \textbf{0.0126} & \textbf{0.0131} \\ 
            \midrule
            S4-TF-S-16 & 0.4893 & 0.2326 & 0.2884 & 0.4252 & 4.503E-05 & 1.425E-04 & 0.0224 & 0.0244 & 0.0249 & 0.0300 \\ 
            S4-TF-L-16 & \textbf{0.4312} & 0.2054 & 0.2331 & 0.3490 & 3.777E-05 & 1.112E-04 & 0.0201 & 0.0233 & 0.0186 & 0.0239 \\ 
            \midrule
            GB-COMP & 0.5823 & 0.2987 & 0.2577 & \textbf{0.1850} & 1.755E-05 & 3.033E-05 & 0.0517 & 0.0635 & 0.1049 & 0.0716 \\ 
            \midrule
            GB-DIST-MLP & 1.1569 & 0.4090 & 0.9312 & 0.7479 & 1.067E-04 & 2.300E-04 & 0.0564 & 0.0463 & 0.2679 & 0.1205 \\ 
            GB-DIST-RNL & 1.1771 & 0.4236 & 1.0591 & 0.7581 & 4.360E-05 & 5.624E-05 & 0.0623 & 0.0496 & 0.2744 & 0.1491 \\ 
            \midrule
            GB-FUZZ-MLP & 1.0794 & 0.3015 & 0.8220 & 0.6536 & 1.372E-05 & 1.097E-05 & 0.0489 & 0.0380 & 0.2096 & 0.1124 \\ 
            GB-FUZZ-RNL & 1.1020 & 0.3110 & 0.7460 & 0.5091 & 2.406E-05 & 3.058E-05 & 0.0500 & 0.0323 & \underline{0.3138} & 0.1571 \\ 
            \midrule
            \midrule
        \end{tabular}
    }
    \vspace{-0.0cm}
    \caption{Overall L1+MR-STFT loss across device type for non parametric models}
    \label{tab:other_fx} \vspace{0.2cm}
\end{table*}

% 1.0239	0.7904
% 0.8909	0.7308
% 0.7582	0.3012
% 0.7246	0.2537
% 0.6904	0.2625
% 0.6461	0.2418
% 0.7573	0.3142
% 0.6390	0.2350
% 0.5793	0.2272
% 0.5237	0.2008
% 0.5390	0.2106
% 0.5097	0.2029
% 0.6026	0.2454
% 0.5307	0.2146
% 0.6947	0.2705
% 0.6579	0.2514
% 0.6289	0.2674
% 0.5950	0.2521
% 0.6273	0.2655
% 0.5757	0.2395
% 0.5393	0.2276
% 0.4868	0.2067
% 0.5500	0.2659
% 0.5109	0.2349
% 0.5385	0.2209
% 0.4867	0.2072
% 0.5699	0.2523
% 0.4627	0.2269
% 0.4893	0.2326
% 0.4312	0.2054
% 0.5823	0.2987
% 1.1569	0.4090
% 1.1771	0.4236
% 1.0794	0.3015
% 1.1020	0.3110

% 2.6187	3.6474	1.566E-04	3.752E-04	0.1267	0.1437	0.2665	0.3115
% 2.3226	3.7729	8.170E-05	1.439E-04	0.1042	0.1183	0.2399	0.3183
% 0.4986	0.3746	5.412E-05	8.496E-05	0.0502	0.0468	0.1188	0.1130
% 0.4024	0.2837	4.244E-05	6.015E-05	0.0424	0.0420	0.1014	0.1113
% 0.4168	0.3117	4.127E-05	5.422E-05	0.0391	0.0333	0.1097	0.1294
% 0.3248	0.2868	2.546E-05	3.563E-05	0.0334	0.0348	0.0840	0.1303
% 0.5320	0.4165	4.186E-05	3.841E-05	0.0426	0.0389	0.1356	0.1549
% 0.3489	0.2967	2.365E-05	3.187E-05	0.0303	0.0314	0.0873	0.1238
% 0.4497	0.5686	4.408E-05	9.285E-05	0.0349	0.0301	0.0690	0.0636
% 0.3201	0.4353	3.124E-05	7.584E-05	0.0256	0.0258	0.0544	0.0418
% 0.3142	0.3776	3.289E-05	7.271E-05	0.0245	0.0210	0.0585	0.0519
% 0.2860	0.3367	2.188E-05	5.471E-05	0.0262	0.0300	0.0555	0.0831
% 0.3725	0.3766	3.887E-05	5.643E-05	0.0252	0.0213	0.0892	0.1102
% 0.4338	0.8216	6.768E-05	1.846E-04	0.0270	0.0310	0.0757	0.1240
% 0.3742	0.3674	1.566E-05	2.600E-05	0.0374	0.0397	0.1126	0.1424
% 0.3337	0.3482	8.867E-06	1.504E-05	0.0363	0.0383	0.0879	0.1341
% 0.3101	0.3311	1.587E-05	3.820E-05	0.0300	0.0292	0.0795	0.1371
% 0.3155	0.3339	1.436E-05	2.681E-05	0.0313	0.0328	0.0646	0.1229
% 0.3582	0.3970	2.080E-05	3.638E-05	0.0296	0.0322	0.0842	0.1743
% 0.3056	0.3099	1.047E-05	2.048E-05	0.0284	0.0308	0.0613	0.0827
% 0.3205	0.3834	2.016E-05	4.763E-05	0.0293	0.0277	0.0665	0.0680
% 0.2881	0.3997	3.470E-05	1.039E-04	0.0251	0.0263	0.0337	0.0368
% 0.3183	0.3734	2.869E-05	7.653E-05	0.0301	0.0340	0.0666	0.0816
% 0.3067	0.3881	4.108E-05	8.833E-05	0.0259	0.0262	0.0547	0.0756
% 0.3185	0.4586	1.854E-05	4.484E-05	0.0218	0.0212	0.0528	0.0616
% 0.2989	0.4172	3.024E-05	8.663E-05	0.0231	0.0286	0.0326	0.0323
% 0.2452	0.2640	8.715E-06	1.692E-05	0.0241	0.0287	0.0643	0.1184
% 0.1702	0.2169	6.061E-06	8.751E-06	0.0185	0.0241	0.0126	0.0131
% 0.2884	0.4252	4.503E-05	1.425E-04	0.0224	0.0244	0.0249	0.0300
% 0.2331	0.3490	3.777E-05	1.112E-04	0.0201	0.0233	0.0186	0.0239
% 0.2577	0.1850	1.755E-05	3.033E-05	0.0517	0.0635	0.1049	0.0716
% 0.9312	0.7479	1.067E-04	2.300E-04	0.0564	0.0463	0.2679	0.1205
% 1.0591	0.7581	4.360E-05	5.624E-05	0.0623	0.0496	0.2744	0.1491
% 0.8220	0.6536	1.372E-05	1.097E-05	0.0489	0.0380	0.2096	0.1124
% 0.7460	0.5091	2.406E-05	3.058E-05	0.0500	0.0323	0.3138	0.1571

==> TABLES/metrics_comp_od.tex <==
\setlength{\tabcolsep}{4pt}
% \vspace{-0.3cm}
% \renewcommand{\arraystretch}{1}
\begin{table*}[h]
    \scriptsize
    \caption{Metrics}
    \label{tab:metrics_1} 
    \centerline{
        \begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc}
            \midrule
            \midrule
            \multirow{4}{*}{Model}
            & \multicolumn{8}{c}{Comp./Limit.}
            & \multicolumn{8}{c}{Overdrive} \\
            
            \cmidrule(lr){2-9} 
            \cmidrule(lr){10-17} 

            & \multicolumn{2}{c}{Tot. Loss}
            & \multicolumn{2}{c}{MSE}
            & \multicolumn{2}{c}{ESR}
            & \multicolumn{2}{c}{MAPE}
            & \multicolumn{2}{c}{Tot. Loss}
            & \multicolumn{2}{c}{MSE}
            & \multicolumn{2}{c}{ESR}
            & \multicolumn{2}{c}{MAPE} \\
        
            \cmidrule(lr){2-3}
            \cmidrule(lr){4-5}
            \cmidrule(lr){6-7}
            \cmidrule(lr){8-9}
            \cmidrule(lr){10-11}
            \cmidrule(lr){12-13}
            \cmidrule(lr){14-15}
            \cmidrule(lr){16-17}
            
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$ 
            & $\mu$ & $\sigma$ 
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$ \\
            
            \midrule
            LSTM-32 
                & 0.4342 & 0.2120
                & 0.0014 & 0.0015 & 1.1476 & 1.9678 & 10.0284 & 15.6637 
                & \underline{1.3099} & \underline{1.0003}
                & 0.0128 & 0.0226 & \underline{0.1409} & 0.1005 & 3.1173 & 2.2259\\ 
            LSTM-96 
                & 0.4276 & 0.2353
                & 0.0008 & 0.0014 & 0.1302 & 0.2536 & 9.6415 & 14.8017 
                & 0.8932 & 0.6595
                & \underline{0.0130} & \underline{0.0234} & 0.1307 & \underline{0.1495} & \underline{3.4952} & \underline{2.8372}\\ 
            \midrule
            TCN-45-S-16 
                & 0.5869 & 0.2363
                & 0.0010 & 0.0013 & 0.1425 & 0.2479 & 7.2482 & 10.3258 
                & 0.5951 & 0.2727
                & 0.0014 & 0.0025 & 0.0109 & 0.0085 & 1.0496 & 0.3987\\ 
            TCN-45-L-16 
                & \underline{0.5948} & 0.1994
                & 0.0013 & 0.0015 & 0.1535 & 0.2506 & 4.4784 & 2.7258 
                & 0.5490 & 0.2383
                & 0.0012 & 0.0021 & 0.0109 & 0.0071 & 0.9156 & 0.3552\\ 
            TCN-250-S-16 
                & 0.5869 & 0.1820
                & 0.0018 & 0.0012 & 1.1184 & 1.8904 & 2.8743 & 1.5673 
                & 0.5847 & 0.2893
                & 0.0011 & 0.0020 & 0.0073 & 0.0077 & 0.6972 & 0.3116\\ 
            TCN-250-L-16 
                &0.5560 & 0.1830
                & 0.0009 & 0.0013 & 0.1397 & \textbf{0.2421} & 2.2316 & 1.0140 
                & 0.5048 & 0.2196
                & 0.0004 & 0.0005 & 0.0052 & 0.0050 & 0.6079 & 0.2978\\ 
            TCN-2500-S-16 
                & 0.5803 & 0.1695
                & 0.0010 & 0.0013 & 0.1488 & 0.2445 & 2.2346 & 1.1144 
                & 0.6516 & 0.3396
                & 0.0022 & 0.0039 & 0.0142 & 0.0152 & 1.0087 & 0.3017\\ 
            TCN-2500-L-16 
                & 0.5670 & \textbf{0.1533}
                & 0.0019 & \textbf{0.0012} & 1.1394 & 1.9164 & 4.1072 & 1.4555 
                & 0.5268 & 0.2314
                & 0.0007 & 0.0011 & 0.0063 & 0.0037 & 0.6744 & 0.2359\\ 
            \midrule
            TCN-TF-45-S-16 
                & 0.4010 & 0.2161
                & 0.0007 & 0.0014 & 0.1280 & 0.2489 & 1.7339 & 1.2091 
                & 0.5416 & 0.1907
                & 0.0011 & 0.0020 & 0.0074 & 0.0077 & 0.8202 & 0.4289\\ 
            TCN-TF-45-L-16
                & 0.4024 & 0.2272
                & 0.0008 & 0.0014 & 0.1333 & 0.2605 & 1.8696 & 1.5078 
                & 0.4852 & 0.1394
                & 0.0007 & 0.0012 & 0.0052 & 0.0043 & 0.7395 & 0.3766\\ 
            TCN-TF-250-S-16 
                & 0.4085 & 0.2281
                & 0.0014 & 0.0015 & 1.1307 & 1.9325 & 1.9766 & 1.0099 
                & 0.4909 & 0.1793
                & 0.0008 & 0.0015 & 0.0060 & 0.0059 & 0.6006 & 0.2419\\ 
            TCN-TF-250-L-16 
                & 0.3973 & 0.2066
                & 0.0007 & 0.0013 & 0.1295 & 0.2469 & 1.6902 & 1.0365 
                & 0.4631 & 0.1704
                & 0.0006 & 0.0007 & 0.0139 & 0.0219 & 0.6609 & 0.4797\\ 
            TCN-TF-2500-S-16 
                & 0.4275 & 0.2103
                & 0.0014 & 0.0015 & 1.1329 & 1.9462 & 2.4618 & \textbf{0.8350} 
                & 0.5704 & 0.2339
                & 0.0018 & 0.0034 & 0.0107 & 0.0138 & 0.6972 & 0.3683\\ 
            TCN-TF-2500-L-16 
                & 0.4139 & 0.2116
                & 0.0015 & 0.0014 & 1.1351 & 1.9451 & 3.2586 & 1.8440 
                & 0.5077 & 0.2430
                & 0.0007 & 0.0012 & 0.0071 & 0.0062 & 0.6464 & 0.2915\\ 
            \midrule
            GCN-45-S-16 
                & 0.5225 & 0.2011
                & 0.0016 & 0.0014 & 1.1211 & 1.9070 & 3.2337 & 2.3538 
                & 0.6151 & 0.3170
                & 0.0014 & 0.0025 & 0.0096 & 0.0092 & 0.8490 & 0.2406\\ 
            GCN-45-L-16 
                & 0.5195 & 0.1917
                & 0.0015 & 0.0014 & 1.1209 & 1.9038 & 12.2879 & 19.9714 
                & 0.5380 & 0.2388
                & 0.0006 & 0.0008 & 0.0085 & 0.0033 & 0.9796 & 0.5657\\ 
            GCN-250-S-16 
                & 0.4713 & 0.1942
                & 0.0015 & 0.0015 & 1.1318 & 1.9345 & 4.3654 & 3.8233 
                & 0.5956 & 0.3101
                & 0.0013 & 0.0021 & 0.0095 & 0.0078 & 1.0302 & 0.3676\\ 
            GCN-250-L-16 
                & 0.4747 & 0.1899
                & 0.0009 & 0.0013 & 0.1338 & 0.2437 & \underline{15.1684} & \underline{25.4238} 
                & 0.4896 & 0.1955
                & 0.0004 & 0.0006 & 0.0032 & 0.0023 & 0.4814 & 0.1995\\ 
            GCN-2500-S-16 
                & 0.4451 & 0.2069
                & 0.0015 & 0.0015 & 1.1148 & 1.8987 & 2.0670 & 1.1710 
                & 0.6179 & 0.3047
                & 0.0020 & 0.0034 & 0.0139 & 0.0128 & 1.1327 & 0.5433\\ 
            GCN-2500-L-16 
                & 0.4274 & 0.2022
                & 0.0008 & 0.0013 & 0.1310 & 0.2484 & 1.8477 & 1.4107 
                & 0.4909 & 0.1778
                & 0.0008 & 0.0014 & 0.0067 & 0.0047 & 0.5810 & 0.1329\\ 
            \midrule
            GCN-TF-45-S-16 
                & 0.3787 & 0.2319
                & 0.0007 & 0.0014 & 0.1275 & 0.2513 & 1.3131 & 1.2324 
                & 0.5288 & 0.1814
                & 0.0010 & 0.0019 & 0.0078 & 0.0078 & 0.6544 & 0.3717\\ 
            GCN-TF-45-L-16 
                & 0.3783 & 0.2192
                & 0.0008 & 0.0013 & 0.1281 & 0.2481 & 1.3617 & 1.1694 
                & 0.4632 & 0.1573
                & 0.0007 & 0.0013 & 0.0063 & 0.0054 & 0.5852 & 0.2641\\ 
            GCN-TF-250-S-16 
                & 0.3882 & 0.2263
                & 0.0007 & 0.0014 & 0.1290 & 0.2499 & 1.4566 & 1.1838 
                & 0.4789 & 0.1352
                & 0.0007 & 0.0012 & 0.0049 & 0.0046 & 0.5851 & 0.2912\\ 
            GCN-TF-250-L-16 
                &0.3857 & 0.2301
                & 0.0007 & 0.0014 & 0.1280 & 0.2496 & 1.4351 & 1.1979 
                & 0.4436 & 0.1563
                & 0.0005 & 0.0009 & 0.0041 & 0.0034 & 0.5180 & 0.2987\\ 
            GCN-TF-2500-S-16 
                & 0.4006 & 0.2290
                & 0.0014 & 0.0016 & 1.1360 & 1.9511 & 1.8734 & 1.2166 
                & 0.5290 & 0.2227
                & 0.0012 & 0.0022 & 0.0075 & 0.0086 & 0.6486 & 0.3147\\ 
            GCN-TF-2500-L-16 
                & 0.3934 & 0.2335
                & 0.0014 & 0.0015 & 1.1359 & 1.9483 & 1.8991 & 1.1881 
                & 0.4496 & 0.1627
                & 0.0009 & 0.0016 & 0.0066 & 0.0056 & 0.5933 & 0.2261\\ 
            \midrule
            S4-S-16 
                & 0.4623 & 0.1893
                & 0.0009 & 0.0013 & 0.1350 & 0.2478 & 2.6336 & 2.0515 
                & 0.5441 & 0.3122
                & 0.0006 & 0.0010 & 0.0052 & 0.0034 & 0.5730 & \textbf{0.1057}\\ 
            S4-L-16 
                & 0.3839 & 0.2035
                & 0.0007 & 0.0013 & 0.1280 & 0.2482 & 3.9584 & 3.7810 
                & \textbf{0.3964} & \textbf{0.1300}
                & \textbf{0.0002} & \textbf{0.0004} & \textbf{0.0024} & \textbf{0.0019} & \textbf{0.3452} & 0.1783\\ 
            \midrule
            S4-TF-S-16 
                & 0.3933 & 0.2422
                & \underline{0.0073} & \underline{0.0127} & \underline{1.8793} & \underline{2.1798} & 1.8137 & 1.7190 
                & 0.4726 & 0.2321
                & 0.0003 & 0.0006 & 0.0037 & 0.0032 & 0.4122 & 0.1806\\ 
            S4-TF-L-16 
                & \textbf{0.3438} & 0.2119
                & \textbf{0.0007} & 0.0013 & \textbf{0.1252} & 0.2473 & \textbf{1.1346} & 1.1706 
                & 0.4001 & 0.1422
                & 0.0004 & 0.0007 & 0.0033 & 0.0031 & 0.3780 & 0.1940\\ 
            \midrule
            GB-COMP 
                & 0.5823 & \underline{0.2987}
                & 0.0013 & 0.0015 & 0.1811 & 0.2787 & 2.0679 & 1.4270 
                & - & -
                & - & - & - & - & - & -\\
            \midrule
            GB-DIST-MLP
                & - & -
                & - & - & - & - & - & - 
                & 0.8390 & 0.2840
                & 0.0118 & 0.0144 & 0.1401 & 0.0875 & 2.3497 & 0.7576\\
            GB-DIST-RNL 
                & - & - 
                & - & - & - & - & - & - 
                & 0.8291 & 0.1482
                & 0.0101 & 0.0119 & 0.1289 & 0.0765 & 2.3810 & 0.5619\\
            \midrule
            GB-FUZZ-MLP 
                & - & - 
                & - & - & - & - & - & - 
                & 0.8500 & 0.2238
                & 0.0079 & 0.0079 & 0.1232 & 0.1061 & 2.1846 & 0.7759\\ 
            GB-FUZZ-RNL 
                & - & - 
                & - & - & - & - & - & - 
                & 0.8636 & 0.2542
                & 0.0104 & 0.0121 & 0.1339 & 0.0850 & 2.6550 & 0.5336\\  
            \midrule
        \end{tabular}
    }
    % \vspace{0.2cm}
\end{table*}

==> TABLES/metrics_dist_fuzz.tex <==
\setlength{\tabcolsep}{4pt}
% \vspace{-0.3cm}
% \renewcommand{\arraystretch}{1}
\begin{table*}[h]
    \scriptsize
    \caption{Metrics}
    \label{tab:metrics_1} 
    \centerline{
        \begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
            \midrule
            \midrule
            \multirow{4}{*}{Model}
            & \multicolumn{8}{c}{Distortion}
            & \multicolumn{8}{c}{Fuzz} \\
            % & \multicolumn{6}{c}{Overall} \\
            
            \cmidrule(lr){2-9} 
            \cmidrule(lr){10-17}
            
            & \multicolumn{2}{c}{Tot. Loss}
            & \multicolumn{2}{c}{MSE}
            & \multicolumn{2}{c}{ESR}
            & \multicolumn{2}{c}{MAPE}
            & \multicolumn{2}{c}{Tot. Loss}
            & \multicolumn{2}{c}{MSE}
            & \multicolumn{2}{c}{ESR}
            & \multicolumn{2}{c}{MAPE} \\
            
            \cmidrule(lr){2-3}
            \cmidrule(lr){4-5}
            \cmidrule(lr){6-7}
            \cmidrule(lr){8-9}
            \cmidrule(lr){10-11}
            \cmidrule(lr){12-13}
            \cmidrule(lr){14-15}
            \cmidrule(lr){16-17}
            
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$ 
            & $\mu$ & $\sigma$ 
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$ \\
            
            \midrule
            LSTM-32 
                & 1.0956 & 0.6605
                & 0.0260 & 0.0411 & \underline{1.2749} & 1.5988 & 7.0533 & 5.4401 
                & 1.2560 & 0.9954
                & 0.0097 & 0.0126 & 0.3682 & 0.4340 & 7.1633 & 7.5367 \\
                % & 0.0125 & 0.0236 & \underline{0.7329} & 1.2564 & 6.8406 & 8.5900\\
            LSTM-96 
                & 1.0873 & \underline{0.8546}
                & 0.0229 & 0.0410 & 0.3959 & 0.4337 & 3.8596 & 2.3782 
                & 1.1554 & \underline{1.0093}
                & 0.0088 & 0.0116 & 0.3487 & 0.4022 & 7.6692 & 8.1115 \\
                % & 0.0114 & 0.0233 & 0.2514 & 0.3212 & 6.1664 & 8.1770\\
            \midrule
            TCN-45-S-16 
                & 0.9274 & 0.2865
                & 0.0189 & 0.0339 & 0.3383 & 0.3496 & 5.1188 & 2.7317 
                & 0.9233 & 0.3039
                & 0.0062 & 0.0053 & 0.1561 & 0.1494 & 6.7955 & 5.9145 \\
                % & 0.0069 & 0.0171 & 0.1619 & 0.2360 & 5.0530 & 6.0178\\
            TCN-45-L-16 
                & 0.9708 & 0.2210
                & 0.0209 & 0.0349 & 0.3726 & 0.3583 & 6.5871 & 3.4021 
                & 0.7839 & 0.1655
                & 0.0036 & 0.0045 & 0.0707 & 0.0223 & 4.0330 & 2.4216 \\
                % & 0.0068 & 0.0179 & 0.1519 & 0.2417 & 4.0035 & 3.0630\\
            TCN-250-S-16 
                & 0.8565 & 0.3099
                & 0.0173 & 0.0319 & 0.2899 & 0.3376 & 3.6665 & 2.4780 
                & 0.7335 & 0.2515
                & 0.0029 & 0.0038 & 0.0538 & 0.0340 & 3.2885 & 2.6089 \\
                % & 0.0058 & 0.0160 & 0.3674 & 0.9750 & 2.6316 & 2.1247\\
            TCN-250-L-16 
                & 0.8594 & 0.2764
                & 0.0168 & 0.0302 & 0.3757 & 0.3802 & 6.4528 & 4.7542 
                & 0.6640 & 0.1893
                & 0.0024 & 0.0039 & 0.0362 & 0.0280 & 1.9113 & 0.9290 \\
                % & 0.0051 & 0.0153 & 0.1392 & 0.2516 & 2.8009 & 3.1706\\
            TCN-2500-S-16 
                & 0.9248 & 0.2849
                & 0.0200 & 0.0310 & 1.0850 & 1.5726 & 13.3287 & 18.5709 
                & 0.8723 & 0.3959
                & 0.0048 & 0.0041 & 0.1404 & 0.1485 & 6.7941 & \underline{8.9978} \\
                % & 0.0070 & 0.0162 & 0.3471 & 0.8412 & 5.8415 & 10.5035\\
            TCN-2500-L-16 
                & 0.8162 & 0.2914
                & 0.0182 & 0.0339 & 0.3250 & 0.3682 & 3.5386 & 2.5631 
                & 0.6460 & 0.2202
                & 0.0031 & 0.0037 & 0.0600 & 0.0340 & 1.9949 & 0.6146 \\
                % & 0.0060 & 0.0169 & 0.3826 & 0.9904 & 2.5788 & 1.9367\\
            \midrule
            TCN-TF-45-S-16 
                & 0.7701 & 0.1957
                & 0.0092 & 0.0162 & 0.1966 & 0.1885 & 2.8666 & 2.0091 
                & 0.6045 & 0.2072
                & 0.0012 & 0.0011 & 0.0301 & 0.0188 & 1.6555 & 1.3187 \\
                % & 0.0030 & 0.0082 & 0.0905 & 0.1605 & 1.7691 & 1.4315\\
            TCN-TF-45-L-16 
                & 0.7083 & 0.1877
                & 0.0070 & 0.0124 & 0.1481 & 0.1384 & 2.5797 & 1.7652 
                & 0.4990 & 0.1659
                & 0.0008 & 0.0008 & 0.0202 & 0.0061 & 0.9399 & 0.5128 \\
                % & 0.0023 & 0.0063 & 0.0767 & 0.1478 & 1.5322 & 1.3202\\
            TCN-TF-250-S-16 
                & 0.7130 & 0.2154
                & 0.0078 & 0.0140 & 0.1509 & 0.1530 & 2.6239 & 1.5171 
                & 0.5435 & 0.1582
                & 0.0010 & 0.0009 & 0.0262 & 0.0170 & 1.0988 & 0.6014 \\
                % & 0.0027 & 0.0070 & 0.3284 & 0.9919 & 1.5750 & \textbf{1.1825}\\
            TCN-TF-250-L-16 
                & 0.6665 & 0.2191
                & 0.0060 & 0.0106 & 0.1384 & 0.1231 & \textbf{2.2852} & 1.5830 
                & 0.5120 & 0.1832
                & 0.0019 & 0.0016 & 0.0853 & 0.1229 & 1.3378 & 1.2524 \\
                % & 0.0023 & 0.0053 & 0.0918 & 0.1446 & 1.4935 & 1.2019\\
            TCN-TF-2500-S-16 
                & 0.7524 & \textbf{0.1508}
                & 0.0061 & 0.0099 & 0.1529 & 0.1324 & 3.0458 & 1.8356 
                & 0.6600 & 0.3208
                & 0.0016 & \textbf{0.0007} & 0.0522 & 0.0293 & 2.7795 & 3.0593 \\
                % & 0.0027 & 0.0052 & 0.3372 & 0.9946 & 2.2461 & 1.9002\\
            TCN-TF-2500-L-16 
                & 0.6422 & 0.1813
                & \textbf{0.0025} & \textbf{0.0038} & \textbf{0.0760} & \textbf{0.0672} & 2.3227 & \textbf{1.0536} 
                &  0.5588 & 0.2390
                & 0.0029 & 0.0008 & 0.1122 & 0.0696 & 1.4733 & 0.9598 \\
                % & \textbf{0.0019} & \textbf{0.0021} & 0.3326 & 0.9945 & 1.9252 & 1.4526\\
            \midrule
            GCN-45-S-16 
                & 0.8718 & 0.3182
                & 0.0189 & 0.0354 & 0.3289 & 0.3722 & 4.3164 & 3.3768 
                & 0.7694 & 0.1622
                & 0.0033 & 0.0047 & 0.0558 & 0.0310 & 3.4175 & 1.6974 \\
                % & 0.0063 & 0.0177 & 0.3789 & 0.9834 & 2.9542 & 2.3940\\
            GCN-45-L-16 
                & 0.8502 & 0.3146
                & 0.0200 & 0.0373 & 0.3308 & 0.3940 & 4.0342 & 2.5898 
                & 0.7237 & \textbf{0.1533}
                & 0.0047 & 0.0043 & 0.1095 & 0.0842 & 3.0313 & 1.2522 \\
                % & 0.0067 & 0.0187 & 0.3924 & 0.9801 & 5.0833 & 10.0618\\
            GCN-250-S-16 
                & 0.8138 & 0.3170
                & 0.0182 & 0.0344 & 0.2791 & 0.3719 & 4.1215 & 2.7158 
                & 0.6350 & 0.2072
                & 0.0024 & 0.0039 & 0.0361 & 0.0279 & 2.2064 & 1.1266 \\
                % & 0.0058 & 0.0172 & 0.3641 & 0.9988 & 2.9309 & 2.5903\\
            GCN-250-L-16 
                & 0.7838 & 0.3312
                & 0.0176 & 0.0335 & 0.2726 & 0.3536 & 3.9375 & 2.8419 
                & 0.6320 & 0.2243
                & 0.0023 & 0.0035 & 0.0412 & 0.0328 & 1.5179 & 0.8166 \\
                % & 0.0053 & 0.0169 & 0.1109 & 0.2262 & 5.5071 & \underline{12.9148}\\
            GCN-2500-S-16 
                & 0.8475 & 0.2696
                & 0.0179 & 0.0328 & 0.2847 & 0.3619 & 3.8666 & 2.6794 
                & 0.5986 & 0.1842
                & 0.0025 & 0.0038 & 0.0526 & 0.0386 & 2.0706 & 0.7846 \\
                % & 0.0060 & 0.0173 & 0.3668 & 0.9796 & 2.3132 & 1.6903\\
            GCN-2500-L-16 
                & 0.7734 & 0.2870
                & 0.0155 & 0.0299 & 0.2604 & 0.3010 & 3.7853 & 2.6634 
                & 0.6112 & 0.1980
                & 0.0014 & 0.0018 & 0.0420 & 0.0370 & 1.6628 & 0.9648 \\
                % & 0.0054 & 0.0173 & 0.1305 & 0.2495 & 2.0239 & 1.9314\\
            \midrule
            GCN-TF-45-S-16 
                & 0.7110 & 0.2228
                & 0.0087 & 0.0158 & 0.1716 & 0.1749 & 2.5546 & 1.6764 
                & 0.5386 & 0.2208
                & 0.0009 & 0.0007 & 0.0199 & 0.0171 & 1.0085 & 0.7863 \\
                % & 0.0028 & 0.0076 & 0.0793 & 0.1505 & 1.5406 & 1.3419\\
            GCN-TF-45-L-16 
                & 0.6605 & 0.2377
                & 0.0072 & 0.0147 & 0.1453 & 0.1426 & 2.2676 & 1.5591 
                & 0.4452 & 0.1595
                & 0.0007 & 0.0009 & 0.0168 & 0.0126 & 0.8965 & 0.6512 \\
                % & 0.0026 & 0.0067 & 0.0824 & 0.1475 & 1.4435 & 1.2826\\
            GCN-TF-250-S-16 
                & 0.7005 & 0.2523
                & 0.0073 & 0.0146 & 0.1391 & 0.1526 & 2.5102 & 1.5732 
                & 0.6323 & 0.3734
                & 0.0008 & 0.0009 & 0.0208 & 0.0191 & 1.1752 & 0.8332 \\
                % & 0.0030 & 0.0074 & 0.0948 & 0.1497 & 1.9687 & 1.9196\\
            GCN-TF-250-L-16 
                & 0.6579 & 0.2604
                & 0.0059 & 0.0108 & 0.1384 & 0.1283 & 2.3073 & 1.5042 
                & 0.5564 & 0.2689
                & 0.0008 & 0.0009 & 0.0221 & 0.0194 & 0.9582 & 0.5849 \\
                % & 0.0023 & 0.0058 & 0.0802 & \textbf{0.1427} & 1.6105 & 1.4593\\
            GCN-TF-2500-S-16 
                & 0.7034 & 0.2127
                & 0.0071 & 0.0135 & 0.1925 & 0.2487 & 2.8877 & 1.8449 
                & 0.5209 & 0.1859
                & 0.0014 & 0.0010 & 0.0249 & 0.0197 & 1.1253 & 0.7062 \\
                % & 0.0031 & 0.0073 & 0.3338 & 0.9989 & 1.8308 & 1.4181\\
            GCN-TF-2500-L-16 
                & 0.6493 & 0.2362
                & 0.0092 & 0.0122 & 0.9928 & \underline{1.7508} & 3.7707 & 3.5123 
                & 0.4547 & 0.1667
                & 0.0015 & 0.0009 & 0.0426 & 0.0148 & 1.2048 & 0.5087 \\
                % & 0.0033 & 0.0066 & 0.5445 & \underline{1.2898} & 1.8670 & 2.0803\\
            \midrule
            S4-S-16 
                & 0.7422 & 0.2931
                & 0.0199 & 0.0382 & 0.3063 & 0.4179 & 4.0564 & 3.5080 
                & 0.5309 & 0.2030
                & 0.0016 & 0.0022 & 0.0314 & 0.0117 & 1.3552 & 0.5474 \\
                % & 0.0058 & 0.0191 & 0.1195 & 0.2493 & 2.1546 & 2.2865\\
            S4-L-16 
                & 0.6490 & 0.3136
                & 0.0314 & 0.0618 & 0.4047 & 0.6553 & 3.6234 & 3.1710 
                & 0.4217 & 0.1949
                & 0.0013 & 0.0018 & 0.0233 & 0.0126 & 0.9670 & \textbf{0.3052} \\
                % & 0.0084 & 0.0309 & 0.1396 & 0.3545 & 2.2235 & 2.7536\\
            \midrule
            S4-TF-S-16 
                & 0.6588 & 0.2655
                & 0.0114 & 0.0217 & 0.1808 & 0.2402 & 2.3433 & 1.7888 
                & 0.4325 & 0.1798
                & 0.0008 & 0.0009 & 0.0176 & \textbf{0.0032} & \textbf{0.9170} & 0.4074 \\
                % & 0.0050 & 0.0122 & 0.5203 & 1.2742 & 1.3716 & 1.3693\\
            S4-TF-L-16 
                & \textbf{0.5599} & 0.2718
                & 0.0093 & 0.0179 & 0.1443 & 0.2008 & 2.3842 & 1.7099 
                & \textbf{0.4210} & 0.1958
                & \textbf{0.0008} & 0.0009 & \textbf{0.0165} & 0.0090 & 0.9325 & 0.6508 \\
                % & 0.0028 & 0.0089 & \textbf{0.0723} & 0.1567 & \textbf{1.2073} & 1.2350\\
            \midrule
            GB-COMP 
                & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
                % & \textbf{0.0013} & \textbf{0.0015} & 0.1811 & 0.2787 & 2.0679 & 1.4270\\
            \midrule
            GB-DIST-MLP 
                & 1.1898 & 0.2909
                & 0.0449 & 0.0716 & 0.7378 & 0.7091 & 10.3810 & 10.0888 
                & 1.4419 & 0.4511
                & 0.0244 & 0.0159 & \underline{1.0270} & \underline{1.2960} & 9.4706 & 7.4702 \\
                % & \underline{0.0270} & 0.0416 & 0.6349 & 0.8638 & 7.4004 & 7.5631\\
            GB-DIST-RNL 
                & 1.1938 & 0.2956	
                & 0.0445 & 0.0732 & 0.7158 & 0.7320 & 14.6935 & 18.3649 
                & \underline{1.5086} & 0.4901
                & 0.0153 & 0.0120 & 0.4121 & 0.2418 & \underline{12.1773} & 8.4441 \\
                % & 0.0233 & 0.0423 & 0.4189 & 0.4757 & \underline{9.7506} & 11.9285\\
            \midrule
            GB-FUZZ-MLP 
                & 1.1920 & 0.2853
                & 0.0454 & \underline{0.0734} & 0.7443 & 0.7307 & 12.2166 & 10.3128 
                & 1.1962 & 0.3108
                & 0.0068 & 0.0048 & 0.1875 & 0.1015 & 6.0351 & 4.5393 \\
                % & 0.0200 & \underline{0.0429} & 0.3517 & 0.4862 & 6.8121 & 7.3087\\
            GB-FUZZ-RNL 
                & \underline{1.2135} & 0.2823
                & \underline{0.0465} & 0.0728 & 0.7457 & 0.7103 & \underline{15.8424} & \underline{19.6554} 
                & 1.2288 & 0.3109
                & 0.0082 & 0.0064 & 0.2203 & 0.0894 & 8.9507 & 4.0216 \\
                % & 0.0217 & 0.0428 & 0.3667 & 0.4706	& 9.1494 &11.8951\\
            \midrule
            \midrule
    \end{tabular}
    }
    % \vspace{-0.0cm}
    % \vspace{0.2cm}
\end{table*}

==> TABLES/metrics_overall.tex <==
\setlength{\tabcolsep}{4pt}
% \vspace{-0.3cm}
% \renewcommand{\arraystretch}{1}
\begin{table*}[h]
    \scriptsize
    \caption{Metrics}
    \label{tab:metrics_1} 
    \centerline{
        \begin{tabular}{lcc|cc|cc|cc}
            \midrule
            \midrule
            \multirow{4}{*}{Model}
            & \multicolumn{6}{c}{Overall} \\
            
            \cmidrule(lr){2-9}
            
            & \multicolumn{2}{c}{Tot. Loss}
            & \multicolumn{2}{c}{MSE}
            & \multicolumn{2}{c}{ESR}
            & \multicolumn{2}{c}{MAPE} \\
            
            \cmidrule(lr){2-3}
            \cmidrule(lr){4-5}
            \cmidrule(lr){6-7}
            \cmidrule(lr){8-9}
            
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$
            & $\mu$ & $\sigma$ \\
            
            \midrule
            LSTM-32 
                & 1.0239 & \underline{0.7904}$_{[1]}$
                & 0.0125 & 0.0236 & \underline{0.7329}$_{[1]}$ & \underline{1.2564}$_{[3]}$ & 6.8406 & 8.5900\\
            LSTM-96 
                & 0.8909 & \underline{0.7308}$_{[2]}$
                & 0.0114 & 0.0233 & 0.2514 & 0.3212 & 6.1664 & 8.1770\\
            \midrule
            TCN-45-S-16 
                & 0.7582 & 0.3012
                & 0.0069 & 0.0171 & 0.1619 & 0.2360 & 5.0530 & 6.0178\\
            TCN-45-L-16 
                & 0.7246 & 0.2537
                & 0.0068 & 0.0179 & 0.1519 & 0.2417 & 4.0035 & 3.0630\\
            TCN-250-S-16 
                & 0.6904 & 0.2625
                & 0.0058 & 0.0160 & 0.3674 & 0.9750 & 2.6316 & 2.1247\\
            TCN-250-L-16 
                & 0.6461 & 0.2418
                & 0.0051 & 0.0153 & 0.1392 & 0.2516 & 2.8009 & 3.1706\\
            TCN-2500-S-16 
                & 0.7573 & \underline{0.3142}$_{[3]}$
                & 0.0070 & 0.0162 & 0.3471 & 0.8412 & 5.8415 & 10.5035\\
            TCN-2500-L-16 
                & 0.6390 & 0.2350
                & 0.0060 & 0.0169 & 0.3826 & 0.9904 & 2.5788 & 1.9367\\
            \midrule
            TCN-TF-45-S-16 
                & 0.5793 & 0.2272
                & 0.0030 & 0.0082 & 0.0905 & 0.1605 & 1.7691 & 1.4315\\
            TCN-TF-45-L-16 
                & 0.5237 & \textbf{0.2008}$^{[1]}$
                & 0.0023 & 0.0063 & \textbf{0.0767}$^{[2]}$ & 0.1478 & 1.5322 & 1.3202\\
            TCN-TF-250-S-16 
                & 0.5390 & 0.2106
                & 0.0027 & 0.0070 & 0.3284 & 0.9919 & 1.5750 & \textbf{1.1825}$^{[1]}$\\
            TCN-TF-250-L-16 
                & 0.5097 & \textbf{0.2029}$^{[2]}$
                & 0.0023 & 0.0053 & 0.0918 & \textbf{0.1446}$^{[2]}$ & 1.4935 & \textbf{1.2019}$^{[2]}$\\
            TCN-TF-2500-S-16 
                & 0.6026 & 0.2454
                & 0.0027 & \textbf{0.0052}$^{[3]}$ & 0.3372 & 0.9946 & 2.2461 & 1.9002\\
            TCN-TF-2500-L-16 
                & 0.5307 & 0.2146
                & \textbf{0.0019}$^{[2]}$ & \textbf{0.0021}$^{[2]}$ & 0.3326 & 0.9945 & 1.9252 & 1.4526\\
            \midrule
            GCN-45-S-16 
                & 0.6947 & 0.2705
                & 0.0063 & 0.0177 & 0.3789 & 0.9834 & 2.9542 & 2.3940\\
            GCN-45-L-16 
                & 0.6579 & 0.2514
                & 0.0067 & 0.0187 & 0.3924 & 0.9801 & 5.0833 & 10.0618\\
            GCN-250-S-16 
                & 0.6289 & 0.2674
                & 0.0058 & 0.0172 & 0.3641 & 0.9988 & 2.9309 & 2.5903\\
            GCN-250-L-16 
                & 0.5950 & 0.2521
                & 0.0053 & 0.0169 & 0.1109 & 0.2262 & 5.5071 & \underline{12.9148}$_{[1]}$ \\
            GCN-2500-S-16 
                & 0.6273 & 0.2655
                & 0.0060 & 0.0173 & 0.3668 & 0.9796 & 2.3132 & 1.6903\\
            GCN-2500-L-16 
                & 0.5757 & 0.2395
                & 0.0054 & 0.0173 & 0.1305 & 0.2495 & 2.0239 & 1.9314\\
            \midrule
            GCN-TF-45-S-16 
                & 0.5393 & 0.2276
                & 0.0028 & 0.0076 & \textbf{0.0793}$^{[3]}$ & 0.1505 & 1.5406 & 1.3419\\
            GCN-TF-45-L-16 
                & 0.4868 & 0.2067
                & 0.0026 & 0.0067 & 0.0824 & \textbf{0.1475}$^{[3]}$ & \textbf{1.4435}$^{[3]}$ & 1.2826\\
            GCN-TF-250-S-16 
                & 0.5500 & 0.2659
                & 0.0030 & 0.0074 & 0.0948 & 0.1497 & 1.9687 & 1.9196\\
            GCN-TF-250-L-16 
                & 0.5109 & 0.2349
                & \textbf{0.0023}$^{[3]}$ & 0.0058 & 0.0802 & \textbf{0.1427}$^{[1]}$ & 1.6105 & 1.4593\\
            GCN-TF-2500-S-16 
                & 0.5385 & 0.2209
                & 0.0031 & 0.0073 & 0.3338 & 0.9989 & 1.8308 & 1.4181\\
            GCN-TF-2500-L-16 
                & \textbf{0.4867}$^{[3]}$ & 0.2072
                & 0.0033 & 0.0066 & \underline{0.5445}$_{[3]}$ & \underline{1.2898}$_{[1]}$ & 1.8670 & 2.0803\\
            \midrule
            S4-S-16 
                & 0.5699 & 0.2523
                & 0.0058 & 0.0191 & 0.1195 & 0.2493 & 2.1546 & 2.2865\\
            S4-L-16 
                & \textbf{0.4627}$^{[2]}$ & 0.2269
                & 0.0084 & 0.0309 & 0.1396 & 0.3545 & 2.2235 & 2.7536\\
            \midrule
            S4-TF-S-16 
                & 0.4893 & 0.2326
                & 0.0050 & 0.0122 & 0.5203 & \underline{1.2742}$_{[2]}$ & \textbf{1.3716}$^{[2]}$ & 1.3693\\
            S4-TF-L-16 
                & \textbf{0.4312}$^{[1]}$ & \textbf{0.2054}$^{[3]}$
                & 0.0028 & 0.0089 & \textbf{0.0723}$^{[1]}$ & 0.1567 & \textbf{1.2073}$^{[1]}$ & \textbf{1.2350}$^{[3]}$\\
            \midrule
            GB-COMP 
                & 0.5823 & \underline{0.2987}
                & \textbf{0.0013}$^{[1]}$ & \textbf{0.0015}$^{[1]}$ & 0.1811 & 0.2787 & 2.0679 & 1.4270\\
            \midrule
            GB-DIST-MLP 
                & \underline{1.1569}$_{[2]}$ & 0.4090
                & \underline{0.0270}$_{[1]}$ & 0.0416 & \underline{0.6349}$_{[2]}$ & 0.8638 & \underline{7.4004}$_{[3]}$ & 7.5631\\
            GB-DIST-RNL 
                & \underline{1.1771}$_{[1]}$ & 0.4236
                & \underline{0.0233}$_{[2]}$ & \underline{0.0423}$_{[3]}$ & 0.4189 & 0.4757 & \underline{9.7506}$_{[1]}$ & \underline{11.9285}$_{[2]}$\\
            \midrule
            GB-FUZZ-MLP 
                & 1.0794 & 0.3015
                & 0.0200 & \underline{0.0429}$_{[1]}$ & 0.3517 & 0.4862 & 6.8121 & 7.3087\\
            GB-FUZZ-RNL 
                & \underline{1.1020}$_{[3]}$ & 0.3110
                & \underline{0.0217}$_{[3]}$ & \underline{0.0428}$_{[2]}$ & 0.3667 & 0.4706	& \underline{9.1494}$_{[2]}$ & \underline{11.8951}$_{[3]}$\\
            \midrule
            \midrule
    \end{tabular}
    }
    % \vspace{-0.0cm}
    % \vspace{0.2cm}
\end{table*}
